Detection of Illicit Drug Trafficking Events on Instagram: A Deep Multimodal Multilabel Learning Approach

Social media such as Instagram and Twitter have become important platforms for marketing and selling illicit drugs. Detection of online illicit drug trafficking has become critical to combat the online trade of illicit drugs. However, the legal status often varies spatially and temporally; even for the same drug, federal and state legislation can have different regulations about its legality. Meanwhile, more drug trafficking events are disguised as a novel form of advertising commenting leading to information heterogeneity. Accordingly, accurate detection of illicit drug trafficking events (IDTEs) from social media has become even more challenging. In this work, we conduct the first systematic study on fine-grained detection of IDTEs on Instagram. We propose to take a deep multimodal multilabel learning (DMML) approach to detect IDTEs and demonstrate its effectiveness on a newly constructed dataset called multimodal IDTE(MM-IDTE). Specifically, our model takes text and image data as the input and combines multimodal information to predict multiple labels of illicit drugs. Inspired by the success of BERT, we have developed a self-supervised multimodal bidirectional transformer by jointly fine-tuning pretrained text and image encoders. We have constructed a large-scale dataset MM-IDTE with manually annotated multiple drug labels to support fine-grained detection of illicit drugs. Extensive experimental results on the MM-IDTE dataset show that the proposed DMML methodology can accurately detect IDTEs even in the presence of special characters and style changes attempting to evade detection.

==> community.tex <==
\section{Unsupervised Learning for Drug-Dealer Community Detection}
\label{sec:4a}

Community detection from a social network refers to the problem of identifying a cluster of connected vertices forming a fairly independent compartments in a graph or a network \cite{newman2006modularity,newman2004finding}. Detecting drug-dealer community (a.k.a drug trafficking ring) in the real world has been studied by social scientists and criminologists for decades \cite{adler1993wheeling}. Finding the community of drug-dealers and their customers from social media data such as Instagram has only been recently considered (e.g., \cite{li2019machine}). By exploring how the hashtags are connected on Instagram, we make the first step toward revealing the hashtag culture, which might lead to useful hints for online community detection. In other words, the complicated relational characteristics of Instagram hashtags can be discovered through data mining and visualization techniques allowing a deeper understanding of drug-dealer community/cluster found across hashtags.

To demonstrate the feasibility of this idea, we have designed an unsupervised learning method using NetworkX \cite{hagberg2008exploring} - a graph object and a Python language package developed for exploiting and analyzing networks. NetworkX has been widely used for operations on large-scale real-world graphs such as graphs with over 10 million nodes and 100 million edges \cite{hagberg2010hacking}. For the IDDIG dataset we have collected from Instegram, more than 800 posts in our dataset all contains at least one mention of drug-related hashtag (e.g., \#pills, \#psychedelic, \#mdmatherapy, \#mdmatrip, \#lsdtrip, and \#lsdls). All unique hashtags in the corpus represented nodes in the graph. Edges were formed between hashtags if they were mentioned together in the same post. This yielded an undirected drug-related graph which was then analysed by NetworkX. For the task of community detection, we can calculate various graph attributes such as between centrality, adjacency frequency, clustering coefficient, and community ID. The identified communities from a network are often visualized by a tool so-called Sunburst plot (please refer to Fig. \ref{fig:8} for illustrative examples).
